Can We Achieve High-quality Direct Speech-to-Speech Translation without Parallel Speech Data?

Recently proposed two-pass direct speech-to-speech translation (S2ST) models decompose the task into speech-to-text translation (S2TT) and text-to-speech (TTS) within an end-to-end model, yielding promising results. However, the training of these models still relies on parallel speech data, which is extremely challenging to collect. In contrast, S2TT and TTS have accumulated a large amount of data and pretrained models, which have not been fully utilized in the development of S2ST models. Inspired by this, in this paper, we first introduce a composite S2ST model named ComSpeech, which can seamlessly integrate any pretrained S2TT and TTS models into a direct S2ST model. Furthermore, to eliminate the reliance on parallel speech data, we propose a novel training method ComSpeech-ZS that solely utilizes S2TT and TTS data. It aligns representations in the latent space through contrastive learning, enabling the speech synthesis capability learned from the TTS data to generalize to S2ST in a zero-shot manner. Experimental results on the CVSS dataset show that when the parallel speech data is available, ComSpeech surpasses previous two-pass models like UnitY and Translatotron 2 in both translation quality and decoding speed. When there is no parallel speech data, ComSpeech-ZS lags behind \name by only 0.7 ASR-BLEU and outperforms the cascaded models.

==> Figures/figure_overview.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/overview.pdf}
    \caption{Comparison of previous two-pass S2ST Models and our proposed composite S2ST model.}
    \label{fig:overview}
\end{figure}

==> Sections/210_s2st.tex <==
% Speech-to-Speech translation (S2ST) refers to the process of translating speech from a source language into speech in a target language.
Formally, using $S$ to denote the source speech and $T$ to denote the target speech, the S2ST model captures the conditional probability $P(T | S)$. Unfortunately, the training of S2ST model relies on the availability of \textit{parallel speech data}, which is extremely challenging to collect. Therefore, most current S2ST datasets \citep{jia2022cvss, DBLP:conf/interspeech/PopuriCWPAGHL22} are derived from existing speech-to-text translation (S2TT) datasets. Denoting the S2TT dataset as $\mathcal{D}_{\text{S2TT}} = \{(S, Y)\}$, researchers typically employ an external text-to-speech (TTS) model to synthesize the target text $Y$ into target speech $T$, thus creating a three-way parallel S2ST dataset $\mathcal{D}_{\text{S2ST}} = \{(S, Y, T)\}$. 

==> Sections/230_rethinking.tex <==
Two-pass architecture effectively decomposes the S2ST task, where $\mathcal{F}_{\text{enc}}$ and $\mathcal{F}_{\text{dec}}$ perform the S2TT task, and $\mathcal{G}_{\text{enc}}$ and $\mathcal{G}_{\text{dec}}$ handle the TTS task. It not only reduces training complexity through task decomposition, but also avoids error propagation through end-to-end training. However, the current training paradigm typically involves simultaneously training all four modules ($\mathcal{F}_{\text{enc}}$, $\mathcal{F}_{\text{dec}}$, $\mathcal{G}_{\text{enc}}$ and $\mathcal{G}_{\text{dec}}$) using parallel speech data, which proves challenging to collect. This prompts us to contemplate the following two questions:
\begin{enumerate}
    \renewcommand{\labelenumi}{(\arabic{enumi})}
    \item Is it possible to train ($\mathcal{F}_{\text{enc}}$, $\mathcal{F}_{\text{dec}}$) and ($\mathcal{G}_{\text{enc}}$, $\mathcal{G}_{\text{dec}}$) separately using existing S2TT and TTS data, or can we leverage pre-trained S2TT and TTS models directly to help S2ST training?
    \item Moreover, can we achieve zero-shot S2ST solely using S2TT and TTS data, without relying on any parallel speech data?
\end{enumerate}

For the first question, we introduce a more general two-pass S2ST model structure which can amalgamate any S2TT model and TTS model into an S2ST model (Section \ref{sec:model}). For the second question, we achieve representation alignment within the model's representation space through contrastive learning, enabling zero-shot S2ST solely using S2TT and TTS data (Section \ref{sec:training}).

==> Sections/A00_data_process.tex <==

\label{app:data_process}

\paragraph{Data Statistics} The statistical information for all datasets are presented in Table~\ref{tab:data}.

\input{Tables/table_data}

\paragraph{Data Processing}
For the source speech, we convert it to 16000Hz and compute 80-dimensional mel-filterbank features. For the target speech, we convert it to 22050Hz and transform the waveform into mel-spectrograms. Utterance-level and global-level cepstral mean-variance normalization are applied to the source speech and target speech, respectively. For the target text, the S2TT model employs a subword vocabulary of size 6k which is learned on the target text of CVSS. The TTS model employs a phoneme vocabulary of size 70. We follow~\citet{ren2021fastspeech2} to extract the duration, pitch, and energy information of the target speech.
